VividPose: Advancing Stable Video Diffusion for Realistic Human Image Animation

Human image animation involves generating a video from a static image by following a specified pose sequence. Current approaches typically adopt a multi-stage pipeline that separately learns appearance and motion, which often leads to appearance degradation and temporal inconsistencies. To address these issues, we propose VividPose, an innovative end-to-end pipeline based on Stable Video Diffusion (SVD) that ensures superior temporal stability. To enhance the retention of human identity, we propose an identity-aware appearance controller that integrates additional facial information without compromising other appearance details such as clothing texture and background. This approach ensures that the generated videos maintain high fidelity to the identity of human subject, preserving key facial features across various poses. To accommodate diverse human body shapes and hand movements, we introduce a geometry-aware pose controller that utilizes both dense rendering maps from SMPL-X and sparse skeleton maps. This enables accurate alignment of pose and shape in the generated videos, providing a robust framework capable of handling a wide range of body shapes and dynamic hand movements. Extensive qualitative and quantitative experiments on the UBCFashion and TikTok benchmarks demonstrate that our method achieves state-of-the-art performance. Furthermore, VividPose exhibits superior generalization capabilities on our proposed in-the-wild dataset. Codes and models will be available.

==> sections/1_introduction.tex <==
\section{Introduction}

Human image animation is a task to generate dynamic and realistic videos from static human images by following a given sequence of poses. This technology has garnered significant attention due to its wide range of applications across various domains. In social media, it can be used to create engaging and personalized content; in the movie and entertainment industry, it facilitates the production of lifelike character animations; and in online retail, it enhances virtual try-ons by animating mannequins. The ability to animate static images into vivid and coherent videos has immense value, making it a highly explored area in both academic research and practical applications.

With the development of powerful generative models such as Generative Adversarial Networks (GANs) and the more recent Diffusion Models (DMs), human image animation has seen significant advancements. 
1) GAN-based methods~\cite{FOMM,TianRCO0MT21,G3AN,RenLLL20,SiarohinLT0S19,MRAA,YuPCZXL23,ZhangYLX22,TPS,ChanGZE19} typically first predict a flow map from the motion changes in the driving video. Although these methods leverage pixel-level pose transition information, inaccuracies in estimating spatial transformations often result in local deformation artifacts, insufficient appearance details and temporal inconsistencies, further restricting their use in real-world applications.
2) DM-based methods~\cite{DreamPose,DISCO,FollowYourPose,MagicAnimate,AnimateAnyone,PIDM,PoseAnimate,MagicPose} achieve human animation video generation by injecting appearance information from the reference image and pose sequences from the driving video into the diffusion model. Recent methods like AnimateAnyone~\cite{AnimateAnyone}, MagicAnimate~\cite{MagicAnimate}, and MagicPose~\cite{MagicPose} utilize ReferenceNet (a copy of the denoising UNet) to encode multi-scale appearance information, effectively preserving fine-grained details such as background and clothing textures. However, these methods model the appearance information of the entire human image as a whole, neglecting the domain gap between facial features and other details like clothing and background. This often leads to models focusing excessively on clothing textures and background details, while failing to maintain high face identity consistency. Moreover, these approaches typically add temporal layers to a 2D image-based diffusion model and perform multi-stage training to separately learn appearance and temporal dynamics. This often results in inter-frame jitter and temporal inconsistencies. Additionally, the pose conditions used by these methods are derived from 2D estimators.  So the shape of pose sequences cannot be modified to align with the reference image’s body shape, which leads to misalignment and results in inaccurate human body shape generation.

To address above limitations, we propose VividPose, a novel end-to-end pipeline based on Stable Video Diffusion~\cite{SVD} (SVD). Essentially, our proposed VividPose leverages the powerful image-to-video generation capabilities of SVD, significantly enhancing the temporal consistency and smoothness of human animation videos. VividPose predominantly consists of an identity-aware appearance controller to improve face identity retention and a geometry-aware pose controller to accommodate diverse human body shapes and hand effects. These innovations ensure that our approach not only maintains high visual fidelity but also handles a wide range of human poses and appearances effectively.

In specific, VividPose is built on top of SVD, which is known for the excellent video generation capabilities. To enhance human identity retention, we introduce an identity-aware appearance controller that incorporates additional facial information without compromising other appearance details (\eg, clothing texture and background details). We utilize ReferenceNet to encode multi-scale features from the reference image, which are then injected into the denoising UNet via spatial self-attention. Then we use CLIP~\cite{CLIP} to encode high-level features and ArcFace~\cite{ArcFace} to encode face identity features, which are then injected into the UNet through a decoupled cross-attention mechanism. This controller ensures that the generated videos maintain high fidelity to the identity of the human subject, preserving key facial features across different poses. To accommodate diverse human body shapes and hand effects, we propose a geometry-aware pose controller. This controller leverages both dense rendering maps from a 3D parametric human model (\ie, SMPL-X~\cite{SMPLX}) and sparse skeleton maps extracted from a 2D pose estimator (\ie, DWPose~\cite{DWPose}). By establishing geometric correspondence between the reconstructed SMPL-X from the reference image and the SMPL-X-based pose sequences from the driving video, our approach ensures accurate body shape generation in the resulting videos. We use two lightweight encoders to separately encode features from the rendering maps and the skeleton maps. These features are then fused through summation. To avoid disrupting the inherent generative capabilities of SVD during initial training, we use zero convolutions at the end of each encoder. The fused feature is then added to the noise latent before being input into the UNet. This robust framework effectively handles a wide variety of body shapes and dynamic hand movements, ensuring high-quality and consistent animations.

Extensive qualitative and quantitative experiments on the UBCFashion and TikTok benchmarks demonstrate that VividPose achieves state-of-the-art results in terms of \textbf{better temporal consistency}, \textbf{higher visual fidelity} and \textbf{stronger generalization ablility}. Additionally, VividPose exhibits superior performance on our proposed in-the-wild dataset, showcasing its robustness and effectiveness in real-world scenarios. In summary, we make the contributions as follows:

\begin{itemize}
    \item We propose VividPose, a novel end-to-end pipeline based on Stable Video Diffusion, which significantly enhances the temporal consistency and smoothness of human animation videos.
    \item We introduce an identity-aware appearance controller that incorporates additional facial information while preserving other appearance details such as clothing texture. This ensures high fidelity to the identity of the human subject across different poses.
    \item  We propose a geometry-aware pose controller that leverages both dense rendering maps and sparse skeleton maps. This ensures accurate body shape generation and handles a wide variety of body shapes and dynamic hand movements effectively.
\end{itemize}

